Tracking the Trackers: Towards Understanding the Mobile Advertising and Tracking Ecosystem

Third-party services form an integral part of the mobile ecosystem: they allow app developers to add features such as performance analytics and social network integration, and to monetize their apps by enabling user tracking and targeted ad delivery. At present users, researchers, and regulators all have at best limited understanding of this third-party ecosystem. In this paper we seek to shrink this gap. Using data from users of our ICSI Haystack app we gain a rich view of the mobile ecosystem: we identify and characterize domains associated with mobile advertising and user tracking, thereby taking an important step towards greater transparency. We furthermore outline our steps towards a public catalog and census of analytics services, their behavior, their personal data collection processes, and their use across mobile apps.

==> Makefile <==
## Fully automated LaTeX Makefile
## (c) Bernhard Ager 2010
## Released under GPLv3 <http://www.gnu.org/licenses/gpl.txt>
##
## This is supposed to work with no (or at most a few) modifications 
## on any LaTeX source directory as a drop in.
## 
## If you have suggestions for or additions to this Makefile, feel free to
## drop me <bernhard@net.t-labs.tu-berlin.de> a mail. I am especially
## interested in further/better auto-conversion rules for picture formats.
##
## Acknowledgements go to Oliver Hohlfeld for proposing a database to track
## auto-generated pictures.
##
## Hard dependencies: GNU make, sed, grep, rm
## Soft dependencies: the tools to convert to the different formats including
## latex, pdflatex, dvips, pstopdf, eps2pdf, fig2dev, inkscape, wmf2eps, ...


## $(MAIN).tex is assumed to be the main latex file
#MAIN=$(basename $(shell grep -Fl '\documentclass' *.tex))
MAIN=paper

## $(TEXFILES) holds all LaTeX source files. Extend wildcard pattern if you
## are holding tex files in subdirectories or adjust to your needs.
TEXFILES=$(wildcard *.tex)

## $(PICTURES) and $(BIBLIOGRAPHY) try to guess the names of required 
## pictures and bib files. The matching rule is quite primitive and is
## easily confused by clutter in lines with \includegraphics or 
## \bibliography. 
PICTURES=$(shell grep -F '\includegraphics' $(TEXFILES) | \
		grep -v '%.*\\includegraphics' | sed 's/.*{\([^{}]*\)}.*/\1/') \
	$(shell grep -F '\pgfimage' $(TEXFILES) | \
		grep -v '%.*\\pgfimage' | sed 's/.*{\([^{}]*\)}.*/\1/') \
	$(shell grep -F '\pgfdeclareimage' $(TEXFILES) | \
		grep -v '%.*\\pgfdeclareimage' | sed 's/.*{\([^{}]*\)}.*/\1/')

BIBLIOGRAPHY=$(addsuffix .bib, $(shell grep -F '\bibliography{' $(TEXFILES) | \
	grep -v '%.*\\bibliography' | sed 's/.*{\([^{}]*\)}.*/\1/'))

PS_PICTURES=$(addsuffix .eps, $(PICTURES))
PDF_PICTURES=$(addsuffix .pdf, $(PICTURES))

## $(PICTURE_DB) keeps track of which pictures were actually created by
## this Makefile. In the clean target this database is used to remove them.
## You might have some manual work to do if you accidentially remove it.
PICTURE_DB = picture.db
PICTURE_DB_ADD = test -f $(PICTURE_DB) && grep -F "$@" $(PICTURE_DB) || echo "$@" >>$(PICTURE_DB)

PDFTK=/usr/bin/pdftk

## call pdflatex target if you prefer pdflatex over latex, dvips, ps2pdf
#
 all: pdflatex
# all: $(MAIN).pdf
# all: pdflatex $(MAIN).ps $(MAIN).pdf
# all: $(MAIN).pdf

## Detection of changed '\cite'ations is a PITA. Any hints welcome.
pdflatex: $(MAIN).tex $(TEXFILES) $(PDF_PICTURES) $(BIBLIOGRAPHY)
	pdflatex $<
ifneq ($(BIBLIOGRAPHY), )
	bibtex $(MAIN) && pdflatex $< && pdflatex $<
endif
#	test -f $(PDFTK) && $(PDFTK) $(MAIN).pdf output $(MAIN)_out.pdf compress || cp $(MAIN).pdf $(MAIN)_out.pdf

.PHONY: $(MAIN).ps $(MAIN).pdf $(MAIN).dvi

$(MAIN).ps: $(MAIN).dvi
	dvips -z -P pdf -t letter -o $@ $<

$(MAIN).pdf: $(MAIN).ps
	ps2pdf -dSAFER -dNOPLATFONTS -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $< $@

## Detection of changed '\cite'ations is a PITA. Any hints welcome.
$(MAIN).dvi: $(MAIN).tex $(TEXFILES) $(PS_PICTURES) $(MAIN).bbl
	grep '^\\citation' $(MAIN).aux | sort >$(MAIN).oc
	latex $<
	grep '^\\citation' $(MAIN).aux | sort >$(MAIN).nc
	cmp $(MAIN).oc $(MAIN).nc || bibtex $(MAIN) && latex $< && latex $<

$(MAIN).bbl: $(BIBLIOGRAPHY)
	latex $(MAIN).tex
	bibtex $(MAIN).aux || true
	latex $(MAIN).tex

## unfortunately produces broken pictures, fallback to eps and eps2pdf
#%.pdf: %.dia
#	dia --export=$@ $<
#	$(PICTURE_DB_ADD)

%.eps: %.dia
	dia --export=$@ $<
	$(PICTURE_DB_ADD)

%.pdf: %.fig
	fig2dev -L pdf $< $@
	$(PICTURE_DB_ADD)

%.eps: %.fig
	fig2dev -L eps $< $@
	$(PICTURE_DB_ADD)

%.eps: %.jpg
	convert $< $@
	$(PICTURE_DB_ADD)

%.pdf: %.png
	convert $< $@
	$(PICTURE_DB_ADD)

%.pdf: %.svg
	inkscape --export-pdf=$@ $<
	$(PICTURE_DB_ADD)

%.eps: %.svg
	inkscape --export-eps=$@ $<
	$(PICTURE_DB_ADD)

%.eps: %.wmf
	wmf2eps --eps -o $@ $<
	$(PICTURE_DB_ADD)

# this rule requires the R script to plot to the correct file,
# relative to the Makefile!
%.eps: %.R
	R --no-save <$<
	test -f $@
	test $@ -nt $<

## This generic rule should be kept as the last one, so that
## native -> pdf generation takes precedence over native -> eps -> pdf
#%.pdf: %.eps
#	epstopdf --outfile=$@ $<
#	$(PICTURE_DB_ADD)

%.eps: %.pdf
	pdftops -eps $< $@
	$(PICTURE_DB_ADD)

clean:
	rm -f $(MAIN).aux $(MAIN).dvi $(MAIN).log $(MAIN).nav $(MAIN).out \
		$(MAIN).pdf $(MAIN).ps $(MAIN).snm $(MAIN).toc $(MAIN).bbl \
		$(MAIN).blg $(MAIN).oc $(MAIN).nc head.tmp body.tmp
	rm -f $(shell test -f $(PICTURE_DB) && cat $(PICTURE_DB))
	rm -f $(PICTURE_DB)

report-pictures:
	@echo $(PICTURES)


==> data_output/basic_stats.tex <==
\def\totalTrackedApps{{1176}\xspace}

\def\totalFlows{{600880}\xspace}

\def\allDomains{{7784}\xspace}

\def\totalIPs{{25687}\xspace}

\def\totalValidApps{{1022}\xspace}



==> data_output/domain_distribution_per_app_stats.tex <==
\def\domainsNotBrowserApps{{8,028}\xspace}




\def\mozillaPublicSuffixReduction{{58.1~}}



==> data_output/thirdparty_stats.tex <==
\def\thirdPartyServices{{262}\xspace}

\def\totalAdNetworks{{50}\xspace}




\def\percentageAdNetworks{{19.1~}}

\def\totalAnalytics{{70}\xspace}




\def\percentageAnalytics{{26.7~}}

\def\totalVendorAnalytics{{6}\xspace}




\def\percentageVendorAnalytics{{2.3~}}

\def\validAppsAfterFilter{{1,044}\xspace}




\def\percentageAnalyticsFivePercent{{0.0~}}




\def\percentageAnalyticsOnePercent{{0.0~}}

\def\appsUsingAnalyticServices{{0}\xspace}




\def\percentageAppsUsingAnalyticServices{{0.0~}}


